Contrastive Tuning: A Little Help to Make Masked Autoencoders Forget

Masked Image Modeling (MIM) methods, like Masked Autoencoders (MAE), efficiently learn a rich representation of the input. However, for adapting to downstream tasks, they require a sufficient amount of labeled data since their rich features code not only objects but also less relevant image background. In contrast, Instance Discrimination (ID) methods focus on objects. In this work, we study how to combine the efficiency and scalability of MIM with the ability of ID to perform downstream classification in the absence of large amounts of labeled data. To this end, we introduce Masked Autoencoder Contrastive Tuning (MAE-CT), a sequential approach that utilizes the implicit clustering of the Nearest Neighbor Contrastive Learning (NNCLR) objective to induce abstraction in the topmost layers of a pre-trained MAE. MAE-CT tunes the rich features such that they form semantic clusters of objects without using any labels. Notably, MAE-CT does not rely on hand-crafted augmentations and frequently achieves its best performances while using only minimal augmentations (crop & flip). Further, MAE-CT is compute efficient as it requires at most 10% overhead compared to MAE re-training. Applied to large and huge Vision Transformer (ViT) models, MAE-CT excels over previous self-supervised methods trained on ImageNet in linear probing, k-NN and low-shot classification accuracy as well as in unsupervised clustering accuracy. With ViT-H/16 MAE-CT achieves a new state-of-the-art in linear probing of 82.2%.

==> tables/cluster_results_in.tex <==
\begin{table}[h]
\begin{center}
\begin{tabular}{lccc}
Method & {B/16} & {L/16} & {H/16}\\
\hline
MAE & 13.8 (-5.4) & 14.3 (-4.1) & 11.1 (-7.6)\\
MoCo~v3~\cite{chen2021exploring} & 43.0 (4.5) & - & - \\
MSN~\cite{assran2022masked} & \textbf{54.2} (10.4) & 45.4 (4.8) & - \\
iBOT~\cite{zhou2021image} & 50.0 (6.7) & 52.0 (9.0) & - \\
MAE-CT & 35.3 (1.1) & 54.9 (11.0)  & \textbf{58.0} (8.4) \\
MAE-CT$_{aug}$ & 46.2 (4.3) & \textbf{56.9} (10.1) & 54.8 (7.9) \\
\end{tabular}
\end{center}
\caption{Comparison of $k$-means cluster accuracy on ImageNet. Parentheses show the silhouette score w.r.t. the ground truth. }
\label{tab:clustering_metrics}
\end{table}

==> tables/combined.tex <==
\begin{table}[h]
\begin{center}
\begin{tabular}{lcc}
Method & Probing & $k$-NN \\
\hline
%\multicolumn{3}{l}{\textit{end-to-end training}} \\
MAE & 76.0 & 60.6 \\
combined pre-training & \textbf{77.8} & \textbf{66.1} \\
\hline
%\multicolumn{3}{l}{\textit{end-to-end training + contrastive tuning}} \\
combined pre-training + CT$_\text{skip}$ & 79.7 & 75.3\\ 
detached pre-training + CT$_\text{skip}$ & 80.1 & 77.0 \\  
combined pre-training + CT & 80.1  & 76.7\\ 
MAE-CT$_{min}$ & \textbf{80.2} & \textbf{77.4} \\  
\end{tabular}
\end{center}
\caption{ Comparison of combined pre-training of MAE and NNCLR without and with applying CT. CT$_\text{skip}$ reuses the head from combined pre-training directly for CT and "detached pre-training" adds a stop gradient operation before the NNCLR head during pre-training. All experiments use a ViT-L/16. Top: The combined pre-training slightly improves over MAE but is far worse than the sequential MAE-CT. Bottom: Reusing the NNCLR head from combined pre-training for CT ("CT$_\text{skip}$") can be a competitive alternative to initializing a new head on top of frozen encoder features, but is less flexible and overall slightly worse.}
\label{tab:combined}
\end{table}

==> tables/linear_probing_h14.tex <==
\begin{table}[h]
\begin{center}
\begin{tabular}{lccc}
Method & {B/16} & {L/16} & {H/14} \\
\hline
\multicolumn{4}{l}{\textit{Minimal image augmentations}} \\
SimMIM~\cite{xie2022simmim} & 56.7 & - & - \\
MAE~\cite{he2022masked} & 68.0 & 76.0 & 77.2 \\

I-JEPA~\cite{assran2023self} & {72.9} & 77.5 & 79.3 \\
MAE-CT & \textbf{73.5} & \textbf{80.2}  & \textbf{81.2} \\
\hline
\multicolumn{4}{l}{\textit{Extensive image augmentations}} \\
MoCo~v3~\cite{chen2021mocov3} & 76.7 & 77.6 &  79.1 \\
MSN~\cite{assran2022masked} & 77.7 & 77.3 & - \\
iBOT~\cite{zhou2021image} & \textbf{79.5} & 81.0 & - \\
Layer Grafting~\cite{jiang2023layergrafting} & 77.7 & 81.0 & - \\
MAE-CT$_{aug}$ & 76.9  & \textbf{81.5}  & \textbf{82.0} \\
\end{tabular}
\end{center}
\caption{
Linear probing accuracy on ImageNet. 
MAE-CT outperforms other methods in the setting of minimal image augmentations.
When using extensive image augmentations, 
self-distillation ID methods are able to use the limited parameters in a ViT-B/16 more efficiently. Due to the superior scaling ability, MAE-CT$_{aug}$ outperforms other methods for ViT-L/16 and ViT-H/14.
}
\label{tab:linear_probing}
\end{table}
